Efficient Serverless Cold Start: Reducing Library Loading Overhead by Profile-guided Optimization

Serverless computing abstracts away server management, enabling automatic scaling, efficient resource utilization, and cost-effective pricing models. However, despite these advantages, it faces the significant challenge of cold-start latency, adversely impacting end-to-end performance. Our study shows that many serverless functions initialize libraries that are rarely or never used under typical workloads, thus introducing unnecessary overhead. Although existing static analysis techniques can identify unreachable libraries, they fail to address workload-dependent inefficiencies, resulting in limited performance improvements. To overcome these limitations, we present SLIMSTART, a profile-guided optimization tool designed to identify and mitigate inefficient library usage patterns in serverless applications. By leveraging statistical sampling and call-path profiling, SLIMSTART collects runtime library usage data, generates detailed optimization reports, and applies automated code transformations to reduce cold-start overhead. Furthermore, SLIMSTART integrates seamlessly into CI/CD pipelines, enabling adaptive monitoring and continuous optimizations tailored to evolving workloads. Through extensive evaluation across three benchmark suites and four real-world serverless applications, SLIMSTART achieves up to a 2.30X speedup in initialization latency, a 2.26X improvement in end-to-end latency, and a 1.51X reduction in memory usage, demonstrating its effectiveness in addressing cold-start inefficiencies and optimizing resource utilization.

==> figures/arch_v2.tex <==
% Gradient Info
  
\tikzset {_m41pz3es6/.code = {\pgfsetadditionalshadetransform{ \pgftransformshift{\pgfpoint{89.1 bp } { -108.9 bp }  }  \pgftransformscale{1.32 }  }}}
\pgfdeclareradialshading{_as0522kn9}{\pgfpoint{-72bp}{88bp}}{rgb(0bp)=(1,1,1);
rgb(0bp)=(1,1,1);
rgb(25bp)=(0,0,0);
rgb(400bp)=(0,0,0)}
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,288); %set diagram left start at 0, and has height of 288

%Shape: Rectangle [id:dp02966369271856162] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (122.16,67.18) -- (446.56,67.18) -- (446.56,226) -- (122.16,226) -- cycle ;
%Shape: Rectangle [id:dp42777109499200994] 
\draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (115.42,61.63) -- (439.67,61.63) -- (439.67,220.45) -- (115.42,220.45) -- cycle ;
%Shape: Rectangle [id:dp14345804538605234] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (108.66,55.17) -- (433.22,55.17) -- (433.22,214) -- (108.66,214) -- cycle ;
%Rounded Rect [id:dp1650923300185423] 
\draw  [fill={rgb, 255:red, 179; green, 177; blue, 177 }  ,fill opacity=0.34 ] (117.98,108.86) .. controls (117.98,95.92) and (128.47,85.44) .. (141.4,85.44) -- (257.25,85.44) .. controls (270.18,85.44) and (280.67,95.92) .. (280.67,108.86) -- (280.67,179.12) .. controls (280.67,192.05) and (270.18,202.53) .. (257.25,202.53) -- (141.4,202.53) .. controls (128.47,202.53) and (117.98,192.05) .. (117.98,179.12) -- cycle ;
%Shape: Rectangle [id:dp6313066767272024] 
\draw  [fill={rgb, 255:red, 126; green, 121; blue, 121 }  ,fill opacity=0.49 ] (134.47,105.61) -- (264.86,105.61) -- (264.86,125) -- (134.47,125) -- cycle ;

%Shape: Rectangle [id:dp6687699692927662] 
\draw  [fill={rgb, 255:red, 126; green, 121; blue, 121 }  ,fill opacity=0.49 ] (134.41,135.54) -- (264.8,135.54) -- (264.8,154.92) -- (134.41,154.92) -- cycle ;

%Straight Lines [id:da4857165574425293] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (198.82,125.68) -- (198.82,135.88) ;

%Rounded Rect [id:dp7453831382833307] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (134.41,169.48) .. controls (134.41,166.14) and (137.12,163.43) .. (140.47,163.43) -- (257.81,163.43) .. controls (261.16,163.43) and (263.87,166.14) .. (263.87,169.48) -- (263.87,187.64) .. controls (263.87,190.98) and (261.16,193.69) .. (257.81,193.69) -- (140.47,193.69) .. controls (137.12,193.69) and (134.41,190.98) .. (134.41,187.64) -- cycle ;


%Rounded Rect [id:dp26598136616568957] 
\draw  [fill={rgb, 255:red, 212; green, 212; blue, 212 }  ,fill opacity=0.29 ] (286.74,118.16) .. controls (286.74,109.94) and (293.4,103.28) .. (301.62,103.28) -- (409.78,103.28) .. controls (418,103.28) and (424.67,109.94) .. (424.67,118.16) -- (424.67,162.82) .. controls (424.67,171.04) and (418,177.7) .. (409.78,177.7) -- (301.62,177.7) .. controls (293.4,177.7) and (286.74,171.04) .. (286.74,162.82) -- cycle ;
%Shape: Rectangle [id:dp8287452736307304] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.45 ] (294.67,123.9) -- (415.67,123.9) -- (415.67,141.04) -- (294.67,141.04) -- cycle ;

%Shape: Rectangle [id:dp9515655674006234] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.45 ] (294.67,149.17) -- (414.67,149.17) -- (414.67,166.31) -- (294.67,166.31) -- cycle ;


%Shape: Rectangle [id:dp6079906180970955] 
\draw   (2.33,91.9) -- (71.76,91.9) -- (71.76,154.58) -- (2.33,154.58) -- cycle ;

%Striped Right Arrow [id:dp6592967993519521] 
\draw   (74.9,141.56) -- (100.18,141.26) -- (100.16,137.69) -- (108.14,144.72) -- (100.24,151.94) -- (100.22,148.38) -- (74.93,148.68) -- cycle ;\draw   (71.33,141.6) -- (72.05,141.59) -- (72.08,148.71) -- (71.37,148.72) -- cycle ;\draw   (72.76,141.58) -- (74.18,141.56) -- (74.22,148.69) -- (72.8,148.71) -- cycle ;
%Striped Right Arrow [id:dp8979672249867905] 
\draw   (75.09,119.14) -- (100.52,118.84) -- (100.51,115.28) -- (108.52,122.31) -- (100.58,129.53) -- (100.56,125.97) -- (75.13,126.27) -- cycle ;\draw   (71.53,119.19) -- (72.24,119.18) -- (72.28,126.3) -- (71.57,126.31) -- cycle ;\draw   (72.96,119.17) -- (74.38,119.15) -- (74.42,126.28) -- (73,126.29) -- cycle ;
%Striped Right Arrow [id:dp2530897920602966] 
\draw   (75.3,102.36) -- (100.49,102.07) -- (100.47,98.5) -- (108.42,105.53) -- (100.55,112.75) -- (100.53,109.19) -- (75.34,109.49) -- cycle ;\draw   (71.74,102.41) -- (72.45,102.4) -- (72.49,109.52) -- (71.77,109.53) -- cycle ;\draw   (73.16,102.39) -- (74.59,102.37) -- (74.62,109.5) -- (73.2,109.51) -- cycle ;

%Curve Lines [id:da9510163454973273] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (117.98,179.12) .. controls (94.33,182) and (221.33,332) .. (301.62,177.7) ;
\draw [shift={(301.62,177.7)}, rotate = 117.49] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da6967329384398298] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (555.09,131) .. controls (674.95,121.82) and (669.39,147.74) .. (598.22,180.58) ;
\draw [shift={(597.15,181.07)}, rotate = 335.39] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da957359459162108] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (354.56,103.63) .. controls (356,-71.83) and (-27.67,52.33) .. (141.4,85.44) ;
\draw [shift={(141.4,85.44)}, rotate = 191.08] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Ellipse [id:dp7174788643629915] 
\draw  [fill={rgb, 255:red, 74; green, 74; blue, 74 }  ,fill opacity=1 ] (584.78,181.07) .. controls (584.78,178.21) and (587.55,175.89) .. (590.96,175.89) .. controls (594.38,175.89) and (597.15,178.21) .. (597.15,181.07) .. controls (597.15,183.93) and (594.38,186.26) .. (590.96,186.26) .. controls (587.55,186.26) and (584.78,183.93) .. (584.78,181.07) -- cycle ;
%Shape: Ellipse [id:dp300714212348131] 
\draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=1 ] (570.81,199.12) .. controls (570.81,196.26) and (573.58,193.94) .. (577,193.94) .. controls (580.41,193.94) and (583.18,196.26) .. (583.18,199.12) .. controls (583.18,201.99) and (580.41,204.31) .. (577,204.31) .. controls (573.58,204.31) and (570.81,201.99) .. (570.81,199.12) -- cycle ;
%Shape: Ellipse [id:dp01862250139791266] 
\draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (562.67,218.15) .. controls (562.67,215.29) and (565.43,212.97) .. (568.85,212.97) .. controls (572.26,212.97) and (575.03,215.29) .. (575.03,218.15) .. controls (575.03,221.01) and (572.26,223.33) .. (568.85,223.33) .. controls (565.43,223.33) and (562.67,221.01) .. (562.67,218.15) -- cycle ;
%Shape: Ellipse [id:dp40876354305411167] 
\draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (578.96,218.15) .. controls (578.96,215.29) and (581.73,212.97) .. (585.14,212.97) .. controls (588.56,212.97) and (591.33,215.29) .. (591.33,218.15) .. controls (591.33,221.01) and (588.56,223.33) .. (585.14,223.33) .. controls (581.73,223.33) and (578.96,221.01) .. (578.96,218.15) -- cycle ;
%Straight Lines [id:da7393651982564822] 
\draw    (574.45,204.31) -- (568.85,212.97) ;
%Straight Lines [id:da02912471564092267] 
\draw    (579.98,203.57) -- (585.14,212.97) ;

%Shape: Ellipse [id:dp29849480555899754] 
\draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=1 ] (600.49,199.12) .. controls (600.49,196.26) and (603.26,193.94) .. (606.68,193.94) .. controls (610.09,193.94) and (612.86,196.26) .. (612.86,199.12) .. controls (612.86,201.99) and (610.09,204.31) .. (606.68,204.31) .. controls (603.26,204.31) and (600.49,201.99) .. (600.49,199.12) -- cycle ;
%Shape: Ellipse [id:dp25883938825554775] 
\draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (594.67,218.15) .. controls (594.67,215.29) and (597.44,212.97) .. (600.86,212.97) .. controls (604.27,212.97) and (607.04,215.29) .. (607.04,218.15) .. controls (607.04,221.01) and (604.27,223.33) .. (600.86,223.33) .. controls (597.44,223.33) and (594.67,221.01) .. (594.67,218.15) -- cycle ;
%Shape: Ellipse [id:dp03044093115675084] 
\draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (610.97,218.15) .. controls (610.97,215.29) and (613.74,212.97) .. (617.15,212.97) .. controls (620.57,212.97) and (623.33,215.29) .. (623.33,218.15) .. controls (623.33,221.01) and (620.57,223.33) .. (617.15,223.33) .. controls (613.74,223.33) and (610.97,221.01) .. (610.97,218.15) -- cycle ;
%Straight Lines [id:da9247674537839132] 
\draw    (603.26,203.82) -- (600.86,212.97) ;
%Straight Lines [id:da9945495230746026] 
\draw    (611.69,202.36) -- (617.15,212.97) ;

%Straight Lines [id:da21582368325757684] 
\draw [shading=_as0522kn9,_m41pz3es6]   (586.38,184.55) -- (579.98,194.55) ;
%Straight Lines [id:da49822342770453676] 
\draw    (596.27,184.06) -- (603.55,194.55) ;

%Curve Lines [id:da7159553491584065] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (253.33,199) .. controls (339.9,286.56) and (393.79,259.28) .. (394.33,180.2) ;
\draw [shift={(394.33,179)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Shape: Can [id:dp2060686784013972] 
\draw   (552.22,12.44) -- (552.22,54.44) .. controls (552.22,59.42) and (534.09,63.44) .. (511.72,63.44) .. controls (489.35,63.44) and (471.22,59.42) .. (471.22,54.44) -- (471.22,12.44) .. controls (471.22,7.47) and (489.35,3.44) .. (511.72,3.44) .. controls (534.09,3.44) and (552.22,7.47) .. (552.22,12.44) .. controls (552.22,17.42) and (534.09,21.44) .. (511.72,21.44) .. controls (489.35,21.44) and (471.22,17.42) .. (471.22,12.44) ;

%Rounded Rect [id:dp02451901151613778] 
\draw   (465,140.83) .. controls (465,135.4) and (469.4,131) .. (474.83,131) -- (547.17,131) .. controls (552.6,131) and (557,135.4) .. (557,140.83) -- (557,170.33) .. controls (557,175.76) and (552.6,180.17) .. (547.17,180.17) -- (474.83,180.17) .. controls (469.4,180.17) and (465,175.76) .. (465,170.33) -- cycle ;

%Striped Right Arrow [id:dp1479266193221045] 
\draw   (521.69,73.21) -- (521.5,113.38) -- (531.5,113.42) -- (511.42,129.78) -- (491.5,113.24) -- (501.5,113.28) -- (501.69,73.12) -- cycle ;\draw   (521.74,63.21) -- (521.73,65.21) -- (501.73,65.12) -- (501.74,63.12) -- cycle ;\draw   (521.72,67.21) -- (521.7,71.21) -- (501.7,71.12) -- (501.72,67.12) -- cycle ;
%Shape: Folded Corner [id:dp3687322423160002] 
\draw   (615.2,281.67) -- (466.89,281.67) -- (466.89,232.33) -- (630,232.33) -- (630,266.87) -- cycle -- (615.2,281.67) ; \draw   (630,266.87) -- (618.16,269.83) -- (615.2,281.67) ;
%Striped Right Arrow [id:dp37551234857157034] 
\draw   (523.12,190.38) -- (522.98,219.4) -- (532.98,219.45) -- (512.92,232.15) -- (492.98,219.26) -- (502.98,219.31) -- (503.12,190.29) -- cycle ;\draw   (523.16,180.38) -- (523.16,182.38) -- (503.16,182.29) -- (503.17,180.29) -- cycle ;\draw   (523.15,184.38) -- (523.13,188.38) -- (503.13,188.29) -- (503.15,184.29) -- cycle ;
%Curve Lines [id:da17254182435601928] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (370,104.17) .. controls (343,43.17) and (324,-26.5) .. (471.22,12.44) ;
\draw [shift={(471.22,12.44)}, rotate = 194.82] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (181.33,22) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 1. Sampling}};
% Text Node
\draw (115.33,257.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 2. Collect Call Path}};
% Text Node
\draw (264,258) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 3. Record initialization time}};
% Text Node
\draw (363.33,11) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 4. Send results }};
% Text Node
\draw (113.57,61) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Serverless Function Instance - 1}};
% Text Node
\draw (529,67.2) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 5. Retrieve results} \\{\large and merge}};
% Text Node
\draw (562.56,133.47) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large 6. Generate} \\ {\large CCT}};
% Text Node
\draw (469.22,250) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{99.12pt}\setlength\topsep{0pt}
\begin{center}
{\large 7. generate Report}
\end{center}

\end{minipage}};
% Text Node
\draw (474.94,130) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{46.76pt}\setlength\topsep{0pt}
\begin{center}
{\large \tool{}\\Visualizer}
\end{center}

\end{minipage}};
% Text Node
\draw (485,25) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{36.75pt}\setlength\topsep{0pt}
\begin{center}
{\large cloud}\\{\large storage}
\end{center}

\end{minipage}};
% Text Node
\draw (103.05,123.8) node [anchor=north west][inner sep=0.75pt]  [rotate=-90.81] [align=left] {\textbf{{\large ...}}};
% Text Node
\draw (1.32,105) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{48.66pt}\setlength\topsep{0pt}
\begin{center}
{\large Function \\invocation}
\end{center}

\end{minipage}};
% Text Node
\draw (320.22,106) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large \tool{}}};
% Text Node
\draw (294.63,150.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\normalsize Import Time Recorder}};
% Text Node
\draw (302.05,125.3) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\normalsize Call Path Collector}};
% Text Node
\draw (161.57,88) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Application}};
% Text Node
\draw (156.08,171) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Source code}};
% Text Node
\draw (169.93,137) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Library-n}};
% Text Node
\draw (169.99,108) node [anchor=north west][inner sep=0.75pt]   [align=left] {{\large Library-1}};


\end{tikzpicture}

==> sections/10-acknowledgement.tex <==
\section{Acknowledgement}
\label{acknowledgement}

This material is partly based on work supported by the National Science Foundation award CNS-2006373.

==> sections/8-threats-to-validity.tex <==
% Add extra space to the current page to fit more content
% \enlargethispage{\baselineskip}

\section{Discussion}
\paragraph{\textbf{Implications}}
During our study, we found that newer versions of libraries often incur higher initialization overheads than their predecessors due to escalating complexity over years of development. Tools like \tool{} can help developers pinpoint areas for improvement. Despite efforts by the system community to devise strategies to reduce cold-start time, inefficient code will continue to impact latency-sensitive applications with suboptimal resource usage. Adopting efficient coding practices with tool support, such as that offered by \tool{}, can help mitigate these issues and optimize resource utilization.

\paragraph{\textbf{Limitations}} \tool{} has two limitations: First, the current implementation of \tool{} is written in Python and incurs higher overhead at high-frequency sampling. To reduce the overhead, we will implement \tool{} in the native language, similar to other state-of-the-art Python profilers. Second, \tool{} cannot monitor native code execution. As a glue language, Python often relies on libraries written in native code. However, current \tool{} relies on the Python library to unwind the call stack and reconstruct the call paths. As a result, \tool{} does not collect the call path of native code execution. We will address the issue by collecting native call paths and reconstructing joint native and Python call paths implemented in other Python profilers~\cite{tan2021toward}.


\begin{comment}
    
\paragraph{\textbf{Generalizability Across Languages and Platforms}}  While \tool{} is designed for Python-based serverless applications, the underlying approach—profiling and optimizing library initialization—can be adapted to other programming languages commonly used in serverless platforms, such as Node.js, Java, and Go. \tool{}'s dynamic profiling techniques could be extended to these environments by leveraging language-specific tools, such as the Java Virtual Machine Tool Interface (JVMTI) for Java or V8 Profiler for Node.js. Future iterations of \tool{} will support multi-language profiling.

Although \tool{} was evaluated on AWS Lambda, its design and approach can be generalized to other serverless platforms such as Google Cloud Functions and Microsoft Azure Functions. The cold-start issue is a platform-agnostic challenge~\cite{azure2018coldstart, google2023startupboost}, affecting all serverless environments due to their reliance on ephemeral infrastructure. By adapting to the nuances of different platforms, \tool{}'s profiling framework can provide similar optimizations across various cloud providers.


\section{Threats to validity}
This section outlines potential threats to the validity of our results. 


\textbf{External Validity:} The effectiveness of \tool{}'s optimization guidance depends on the inputs provided to serverless functions during profiling. Different inputs can lead to varying execution paths and library usage. 

\textbf{Internal Validity:} As a statistical profiler, \tool{} relies on the Law of Large Numbers, requiring many samples over time for accuracy. To address this, we tested \tool{} with standard inputs and collected numerous samples by monitoring many serverless function invocations. 

\textbf{Construct Validity:} \tool{} only monitors Python library usage and does not capture native code execution (e.g., C libraries used by Python). This limits its ability to fully capture all sources of cold-start inefficiencies in applications that rely on mixed-language libraries. We plan to extend \tool{} by incorporating native code profiling in future versions. 


\textbf{Conclusion Validity:} The optimizations suggested by \tool{} are guided but not enforced. Developers are responsible for implementing the changes based on the tool’s reports, which introduces variability in how well the optimizations are applied. Incorrect or incomplete implementation could skew the observed performance improvements. 
\end{comment}

==> sections/backup_background.tex <==
\section{Empirical Study and Motivation}
\label{background}
\label{motive}
This section introduces our empirical study and its results, which motivated our work. 

\subsection{Impact of Library Loading on End-to-End Latency}
\begin{figure}[!hbt]
    % \setlength{\belowcaptionskip}{-20pt}
    \includegraphics[width=\linewidth]{figures/libinit_to_e2e_ratio_plot.pdf}
    \caption{Ratio of library Initialization time to  execution time.}
    \label{fig:init_to_e2e}
\end{figure}
To quantify the impact of library initialization on overall execution time, we evaluated a collection of serverless Python applications drawn from existing literature~\cite{yu2024rainbowcake,liu2023faaslight}. Figure \ref{fig:init_to_e2e} presents the library initialization time, execution time, and their respective ratios. The results demonstrate that, for the majority of serverless applications, library initialization contributes to more than 70\% of the total execution time. These findings highlight the critical importance of optimizing library initialization to significantly reduce cold-start latency in serverless Python applications.



\begin{observation}
Library initialization introduces considerable overhead to end-to-end latency during a cold start.

\end{observation}

\subsection{Impact of Library Loading on End-to-End Latency}

\begin{figure}
    % \setlength{\belowcaptionskip}{-15pt}
    \includegraphics[width=\linewidth]{figures/pdf_and_cdf_side_by_side.pdf}
    \caption{PDF plot of serverless applications by the number of handler functions and CDF of entry point invocation frequencies from production trace data.}
    \label{fig:realTrace}
\end{figure}

The invocation patterns of serverless handler functions reveal significant variability in their usage, with a small subset of functions dominating execution. Figure~\ref{fig:realTrace} plots the production traces~\cite{shahrad2020serverless} demonstrating the invocation patterns across handler functions. The PDF plot demonstrates that 54\% of serverless applications include more than one handler function, indicating structural diversity and the potential for varied execution paths across serverless workloads. The CDF plot further illustrates that the first few handler functions account for over 80\% of the cumulative invocation frequency, while higher-ranked functions contribute diminishingly to the total. This steep cumulative growth indicates a strong concentration of invocations on a subset of entry points, while other handler functions are infrequently invoked or unused. While the data does not directly confirm a relationship between entry points and specific library usage, the variability in handler function usage highlights the possibility that not all libraries are required during every invocation, as different entry points may trigger distinct call paths with varying library dependencies. 


%These findings highlight the inefficiency of eagerly initializing all libraries during cold starts, as many libraries may be associated with call paths that are rarely or never executed. By focusing on optimizing library usage for frequently invoked functions, selective or lazy library initialization strategies can significantly reduce cold-start latency.


\begin{observation}
    Serverless applications exhibit highly variable handler function usage, with a few entry points dominating invocations. This variability suggests that different invocations may follow distinct call paths, potentially requiring different subsets of libraries and rendering some library initializations unnecessary during cold starts.
\end{observation}

%Through a thorough manual review of serverless applications, we discover that a significant number of libraries or modules are loaded unnecessarily during serverless function invocation and could be eliminated. This observation aligns with the dynamic nature of serverless workloads, where different invocations can trigger varied execution paths, leading to inconsistent library usage patterns. 

%By leveraging the insights from these plots, selective or lazy library initialization strategies can be employed to reduce cold-start latency, particularly in applications with significant variability in handler function usage.

%However, pinpointing such optimization opportunities within the code is a challenging task.


% \subsection{\textbf{Serverless Cold-start}}

% Figure~\ref{fig:serverless_lifecycle} illustrates the lifecycle of a serverless function. The initial function invocation triggers a cold start, which involves a three-phase initialization process: environment bootstrapping, container initialization, and function setup. Once the function is initialized, it proceeds to execution. Typically, the function container remains active for a predefined \textit{keep-alive} period. Subsequent invocations within this \textit{keep-alive} period result in a warm start, allowing the function to execute without undergoing the re-initialization phases. Upon expiration of the keep-alive period, the container is reclaimed, and any subsequent invocations will trigger a cold start, necessitating the three-phase re-initialization process. The cold start latency is influenced by these three phases:

% \begin{itemize}[leftmargin=*]

%     \item \textbf{Environment initialization} involves setting up the infrastructure environment including setting up network connections, loading configuration files, and starting background processes to provide functionalities such as logging, monitoring, and security enhancements.
%     \item \textbf{Container initialization} entails setting up the runtime environment needed to execute the serverless function. This includes loading the runtime binaries and libraries necessary for the function's execution. The runtime could be based on various programming languages (e.g., Python, Node.js, Java), and this phase ensures that all required dependencies and resources for the runtime are available and configured correctly.
%     \item \textbf{Function initialization} includes loading the actual function code and its dependent libraries into memory. This phase involves running any static initializers and setting up global variables as defined in the function code. It ensures that the function is fully prepared to handle incoming events or requests by completing any necessary setup tasks within the function itself. \textit{This paper addresses the library initialization occurring in this third phase}.
% \end{itemize}

% \begin{figure*}[ht]
%     \centering
%     \begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%     %uncomment if require: \path (0,338); %set diagram left start at 0, and has height of 338
    
%     %Shape: Rectangle [id:dp7228598985848678] 
%     \draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=1 ] (2,117) -- (81,117) -- (81,162.5) -- (2,162.5) -- cycle ;
    
%     %Straight Lines [id:da11892162525354166] 
%     \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ]   (2,90.5) -- (2,117) ;
%     %Straight Lines [id:da7469908554930371] 
%     \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (5.59,100.83) -- (83.67,100.83) ;
%     \draw [shift={(2.59,100.83)}, rotate = 0] [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
    
%     %Straight Lines [id:da419038120139158] 
%     \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ]   (239,90.5) -- (239,117) ;
%     %Straight Lines [id:da3594043421551105] 
%     \draw [color={rgb, 255:red, 128; green, 128; blue, 128 }  ,draw opacity=1 ] [dash pattern={on 4.5pt off 4.5pt}]  (162,100.5) -- (235.69,100.5) ;
%     \draw [shift={(238.69,100.5)}, rotate = 180] [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
    
%     %Shape: Rectangle [id:dp392449362364079] 
%     \draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (281.8,117) -- (338.5,117) -- (338.5,162.5) -- (281.8,162.5) -- cycle ;
    
%     %Shape: Rectangle [id:dp8042873496530669] 
%     \draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (357.6,117) -- (414.3,117) -- (414.3,162.5) -- (357.6,162.5) -- cycle ;
%     %Shape: Rectangle [id:dp7348756538125365] 
%     \draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (434.2,117) -- (490.9,117) -- (490.9,162.5) -- (434.2,162.5) -- cycle ;
    
%     %Straight Lines [id:da44270343053942174] 
%     \draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (339,139) -- (357.8,138.6) ;
%     %Straight Lines [id:da1355226346218903] 
%     \draw [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ] [dash pattern={on 0.84pt off 2.51pt}]  (414.4,139) -- (433.2,138.6) ;
%     %Shape: Rectangle [id:dp07771020416008678] 
%     \draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (81,117) -- (160,117) -- (160,162.5) -- (81,162.5) -- cycle ;
    
%     %Shape: Rectangle [id:dp5354485052452784] 
%     \draw  [fill={rgb, 255:red, 214; green, 210; blue, 211 }  ,fill opacity=1 ] (160,117) -- (239,117) -- (239,162.5) -- (160,162.5) -- cycle ;
    
%     %Straight Lines [id:da09034402375588857] 
%     \draw    (2,162.5) -- (2,189) ;
%     %Straight Lines [id:da9045560811670486] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (5.67,174.03) -- (60.6,174.6) ;
%     \draw [shift={(2.67,174)}, rotate = 0.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%     %Straight Lines [id:da37254282083946166] 
%     \draw    (239,162.5) -- (239,189) ;
%     %Straight Lines [id:da6714608758530558] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (187,174.2) -- (235.67,174.33) ;
%     \draw [shift={(238.67,174.33)}, rotate = 180.15] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%     %Straight Lines [id:da6947074868757468] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (239.6,139) -- (281.6,139) ;
%     %Straight Lines [id:da26777060093988236] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (491.2,139) -- (533.2,139) ;
%     %Straight Lines [id:da18127660808610302] 
%     \draw    (281.78,161.5) -- (281.78,188) ;
%     %Straight Lines [id:da7545283493026116] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (285.4,174.01) -- (339.8,174.2) ;
%     \draw [shift={(282.4,174)}, rotate = 0.2] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%     %Straight Lines [id:da2500348907249126] 
%     \draw    (490.88,161.83) -- (490.88,188.33) ;
%     %Straight Lines [id:da3261416961244765] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (438.2,174.2) -- (487.57,174.64) ;
%     \draw [shift={(490.57,174.67)}, rotate = 180.51] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%     %Shape: Rectangle [id:dp41286511710816054] 
%     \draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (537.33,117) -- (616.33,117) -- (616.33,162.5) -- (537.33,162.5) -- cycle ;
    
%     %Shape: Rectangle [id:dp7696970429706551] 
%     \draw  [fill={rgb, 255:red, 128; green, 128; blue, 128 }  ,fill opacity=1 ] (615.93,117) -- (694.93,117) -- (694.93,162.5) -- (615.93,162.5) -- cycle ;
    
%     %Straight Lines [id:da6744709059176339] 
%     \draw    (537.33,161.8) -- (537.33,188.3) ;
%     %Straight Lines [id:da7673843560401112] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (539.99,172.16) -- (569.8,171.8) ;
%     \draw [shift={(536.99,172.2)}, rotate = 359.3] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%     %Straight Lines [id:da9803328006753196] 
%     \draw    (694.87,161.8) -- (694.87,188.3) ;
%     %Straight Lines [id:da33987559826284564] 
%     \draw  [dash pattern={on 4.5pt off 4.5pt}]  (665.4,172.2) -- (691.55,172.01) ;
%     \draw [shift={(694.55,171.99)}, rotate = 179.59] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
    
%     % Text Node
%     \draw (97.33,95.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {Cold-start};
%     % Text Node
%     \draw (579.97,169) node [anchor=north west][inner sep=0.75pt]   [align=left] {SHUTDOWN};
%     % Text Node
%     \draw (361.35,127.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {Invoke};
%     % Text Node
%     \draw (350.06,169) node [anchor=north west][inner sep=0.75pt]   [align=left] {INVOCATION};
%     % Text Node
%     \draw (77.67,169.8) node [anchor=north west][inner sep=0.75pt]   [align=left] {INITIALIZATION};
%     % Text Node
%     \draw (617.93,118) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{50.35pt}\setlength\topsep{0pt}
%     \begin{center}
%     Extension \\Shutdown
%     \end{center}
    
%     \end{minipage}};
%     % Text Node
%     \draw (541.33,118) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{48.09pt}\setlength\topsep{0pt}
%     \begin{center}
%     Runtime \\Shutdown
%     \end{center}
    
%     \end{minipage}};
%     % Text Node
%     \draw (166,118) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{44.68pt}\setlength\topsep{0pt}
%     \begin{center}
%     Function \\Init
%     \end{center}
    
%     \end{minipage}};
%     % Text Node
%     \draw (88,119) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{43.54pt}\setlength\topsep{0pt}
%     \begin{center}
%     Runtime \\Init
%     \end{center}
    
%     \end{minipage}};
%     % Text Node
%     \draw (437.8,127.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {Invoke};
%     % Text Node
%     \draw (286.45,127.4) node [anchor=north west][inner sep=0.75pt]   [align=left] {Invoke};
%     % Text Node
%     \draw (4,118) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{50.35pt}\setlength\topsep{0pt}
%     \begin{center}
%     Extension \\Init
%     \end{center}
    
%     \end{minipage}};
    
    
%     \end{tikzpicture}
%     \caption{Lifecycle of Serverless Application}
%     \label{fig:serverless_app_lifecycle}
% \end{figure*}


